Measurement of the charge asymmetry in semileptonic Bs decays

We have performed the first direct measurement of the time integrated flavor untagged charge asymmetry in semileptonic Bs decays, Asl(unt), by comparing the decay rate of Bs --> mu+ Ds- nu X, where Ds- --> phi pi- and phi --> K+K-, with the charge-conjugate Bs-bar decay rate. This sample was selected from 1.3/fb of data collected by the D0 experiment in RunII of the Fermilab Tevatron collider. We obtain Asl(unt) = [1.23 +- 0.97(stat) +- 0.17(syst)]*10^-2. Assuming that Delta(M_s)/Gamma_s >> 1 and Delta(Gamma_s)/(2 Gamma_s) < 1, this result can be translated into a measurement on the CP-violating phase in Bs mixing: Delta(Gamma_s)/Delta(M_s)*tan(phi_s) = [2.45 +- 1.93(stat) +- 0.35(syst)]*10^-2.

==> list_of_visitor_addresses_r2.tex <==
% list_of_visitor_addresses_r2.tex                            11/21/06
%
%\bibitem[*]{kurca}
%On leave from IEP SAS Kosice, Slovakia.
\bibitem[*]{alton}
Visitor from Augustana College, Sioux Falls, SD, USA
\bibitem[\dag]{voutilainen}
Visitor from Helsinki Institute of Physics, Helsinki, Finland.
%\bibitem[\ddag]{kozminski}
%Visitor from Lewis University, Romeoville, IL, USA
%
\vskip 0.25cm

